Reparameterization through Spatial Gradient Scaling

Reparameterization aims to improve the generalization of deep neural networks by transforming convolutional layers into equivalent multi-branched structures during training. However, there exists a gap in understanding how reparameterization may change and benefit the learning process of neural networks. In this paper, we present a novel spatial gradient scaling method to redistribute learning focus among weights in convolutional networks. We prove that spatial gradient scaling achieves the same learning dynamics as a branched reparameterization yet without introducing structural changes into the network. We further propose an analytical approach that dynamically learns scalings for each convolutional layer based on the spatial characteristics of its input feature map gauged by mutual information. Experiments on CIFAR-10, CIFAR-100, and ImageNet show that without searching for reparameterized structures, our proposed scaling method outperforms the state-of-the-art reparameterization strategies at a lower computational cost.

==> F-Limitations.tex <==
\section{Limitations}
Spatial gradient scaling can enhance model generalization at a low cost without augmenting training or inference structure. When the optimizer is a linear function of the current and past gradients and weights, spatial gradient scaling has equivalence to $N$-branch structural reparameterization. SGS lacks an interpretation through structural reparameterization for non-linear optimizers, although we can still apply it to scale gradients.
